Opportunities and challenges to study solar neutrinos with a Q-Pix pixel readout

The study of solar neutrinos presents significant opportunities in astrophysics, nuclear physics, and particle physics. However, the low-energy nature of these neutrinos introduces considerable challenges to isolate them from background events, requiring detectors with low-energy threshold, high spatial and energy resolutions, and low data rate. We present the study of solar neutrinos with a kiloton-scale liquid argon detector located underground, instrumented with a pixel readout using the Q-Pix technology. We explore the potential of using volume fiducialization, directional topological information, light signal coincidence and pulse-shape discrimination to enhance solar neutrino sensitivity. We find that discriminating neutrino signals below 5 MeV is very difficult. However, we show that these methods are useful for the detection of solar neutrinos when external backgrounds are sufficiently understood and when the detector is built using low-background techniques. When building a workable background model for this study, we identify {\gamma} background from the cavern walls and from capture of {\alpha} particles in radon decay chains as both critical to solar neutrino sensitivity and significantly underconstrained by existing measurements. Finally, we highlight that the main advantage of the use of Q-Pix for solar neutrino studies lies in its ability to enable the continuous readout of all low-energy events with minimal data rates and manageable storage for further offline analyses.

==> results/light_table.tex <==
\begin{table}[htb]
   \centering
    \begin{tabular}{c|c|c}
        \toprule
        Background scenario              & \makecell{Expected\\B8 CC} & \makecell{Expected\\bkg coincidences} \\
        \midrule
        Baseline Scenario                    & $4.31 \times 10^{3}$       & $\sim 10^{8}$\\
        Low-Bkg Scenario                            & $4.31 \times 10^{3}$       & $\sim 10^{5}$\\
        \hline
        Baseline with LZ constrain                & $4.31 \times 10^{3}$       & $\sim 10^{8}$\\
        Low-Bkg with LZ constrain               & $4.31 \times 10^{3}$       & $\sim 10^{4}$\\
        \hline
        \makecell{Baseline with LZ constrain\\$10^{-1}$ gamma suppression} & $4.31 \times 10^{3}$       & $\sim 10^{8}$\\
        \makecell{Low-Bkg with LZ constrain\\$10^{-1}$ gamma suppression}           & $4.31 \times 10^{3}$       & $\sim 10^{3}$\\
        \bottomrule
    \end{tabular}
    \caption{Expected C8 events and background coincidences under different background scenarios.}
   \label{tab:light}
\end{table}
